Automated Detection of Adverse Drug Reactions in the Biomedical Literature Using Convolutional Neural Networks and Biomedical Word Embeddings

Monitoring the biomedical literature for cases of Adverse Drug Reactions (ADRs) is a critically important and time consuming task in pharmacovigilance. The development of computer assisted approaches to aid this process in different forms has been the subject of many recent works. One particular area that has shown promise is the use of Deep Neural Networks, in particular, Convolutional Neural Networks (CNNs), for the detection of ADR relevant sentences. Using token-level convolutions and general purpose word embeddings, this architecture has shown good performance relative to more traditional models as well as Long Short Term Memory (LSTM) models. In this work, we evaluate and compare two different CNN architectures using the ADE corpus. In addition, we show that by de-duplicating the ADR relevant sentences, we can greatly reduce overoptimism in the classification results. Finally, we evaluate the use of word embeddings specifically developed for biomedical text and show that they lead to a better performance in this task.

==> Makefile <==
all: acl2017.pdf

acl2017.pdf: acl2017.dvi
	dvipdf acl2017.dvi

acl2017.dvi: acl2017.tex acl2017.bib
	latex acl2017.tex && \
	bibtex acl2017.aux && \
	latex acl2017.tex && \
	latex acl2017.tex

clean:
	rm acl2017.aux acl2017.log acl2017.blg acl2017.dvi acl2017.pdf

